ACE: Adversarial Correspondence Embedding for Cross Morphology Motion Retargeting from Human to Nonhuman Characters

Motion retargeting is a promising approach for generating natural and compelling animations for nonhuman characters. However, it is challenging to translate human movements into semantically equivalent motions for target characters with different morphologies due to the ambiguous nature of the problem. This work presents a novel learning-based motion retargeting framework, Adversarial Correspondence Embedding (ACE), to retarget human motions onto target characters with different body dimensions and structures. Our framework is designed to produce natural and feasible robot motions by leveraging generative-adversarial networks (GANs) while preserving high-level motion semantics by introducing an additional feature loss. In addition, we pretrain a robot motion prior that can be controlled in a latent embedding space and seek to establish a compact correspondence. We demonstrate that the proposed framework can produce retargeted motions for three different characters -- a quadrupedal robot with a manipulator, a crab character, and a wheeled manipulator. We further validate the design choices of our framework by conducting baseline comparisons and a user study. We also showcase sim-to-real transfer of the retargeted motions by transferring them to a real Spot robot.

==> algos/train_generator.tex <==
\begin{algorithm}[t] 
\caption{Adversarial Correspondence Embedding} \label{algo:training}
\begin{algorithmic}

\State {G,D $\gets$ randomly initialize generator and discriminator } 
\State {$\pi \gets$ pretrain motion prior }
\While {Update set not enough\sehoon{vague} }
\State {$t \gets 1$ }
\State {$\bar{x}^q_0  \gets$  Initialize robot}
\state {$\xi_i \gets$ randomly sample from dataset}

    \While{$\xi_i$ not \textbf{END}}
        \State {$\bar{x}^p_t \gets \xi_i$? \sehoon{what is $\xi$?}} 
        \State {$\hat{z}_t \gets G(\bar{x}^p_t, \bar{x}^q_{t-1})$ }
        \state {$\hat{x}^q_t \gets \pi(\hat{z}_t, \bar{x}^q_{t-1})$}
        \State {$t \gets t+1$ }

        \State {Update discriminator D }
        \State {Update generator G}
        
    \EndWhile
\EndWhile

\end{algorithmic}
\end{algorithm}


==> paper_text/ACE.tex <==
\section{Adversarial Correspondence Embedding}
In this section, we aim to learn an effective motion retargeting function. Although the problem of motion retargeting has intrinsic ambiguity, we want the retargeted motion to have the following properties. First, the retargeted motion should be naturalistic, which looks plausible on the robot character. Second, the retargeted motion should preserve the key features of the source motion. We approached this problem by designing two loss functions: a naturalness loss $L_{Na}$ and a feature loss $L_{Fea}$. Because it is hard to manually define the naturalness loss, we employ generative adversarial learning~\cite{aberman2020skeleton, villegas2018neural}, which uses a trained discriminator $D$ to measure if the retargeted motions from the generator $G$ are distinguishable from the existing motion dataset. Then we further design a feature loss to match the high-level features of the source and target motions.

\subsection{Problem Formulation}
The original formulation of motion retargeting with Generative Adversarial Network (GAN) learns a generator G to directly map the motion of the source character $\mathbf{x}^h$ into the motion of the target character $\mathbf{x}^r$. However, this is relatively hard to learn effective generator and discriminator networks due to the high dimensional input and output spaces. 

Instead, we leverage our pre-trained motion prior to learning the correspondence in a compact latent space. Our generator (motion retargeting network) $G(\mathbf{x}^h_t, \mathbf{x}^r_{t-1}) \mapsto \mathbf{z}^r_{t-1}$ takes the current human pose $\mathbf{x}^h_t$ and the previous robot motion $\mathbf{x}^r_{t-1}$ to generator the latent variable $\mathbf{z}^r_{t-1}$. Then our discriminator $D(\mathbf{z}^r) \mapsto [0, 1]$ compares the generated variable $\hat{\mathbf{z^r}}$ against the latent variables $\mathbf{z}^r$ in the dataset. 
% This system architecture is also illustrated in the overview figure (Figure XXX).

\subsection{Training of Discriminator}
Therefore, a discriminator D can be trained to distinguish between original latent variables $\mathbf{z}^r$ in the robot motion dataset $\Omega^r$ or generated latent variables $\hat{\mathbf{z}}^r$:
\begin{equation}\label{equ:discriminator_training}
    \argmin_{D}\  \; -\mathbb{E}_{\Omega^r}[log(D(\mathbf{z}^r))] -\mathbb{E}_{\Omega^h}[log(1-D(G(\mathbf{x}^h_t, \mathbf{x}^r_{t-1}) ))].
\end{equation}
However, GAN uses an iterative updating formulation for training the discriminator and the generator, which often causes unstable training dynamics. One reason is non-zero gradients on the manifold of real data samples \cite{mescheder2018training} due to the approximation error in the discriminator. Thus, we incorporate a gradient penalty regularizes used in the other papers~\cite{ASE} to stabilize the training and improve the quality of the training result. This gradient penalty augments the previous discriminator objective as:
\begin{multline} \label{equ: gradient penlty}
    \argmin_{D}\  \; -\mathbb{E}_{\Omega^r}[log(D(\mathbf{z}^r))] -\mathbb{E}_{\Omega^h}[log(1-D(G(\mathbf{x}^h_t, \mathbf{x}^r_{t-1}) ))] \\ 
    + \frac{w^{gp}}{2}\mathbb{E}_{\Omega^r}[||\nabla_\lambda D(\lambda) |_{\lambda=\mathbf{z}^r}   ||^2],
\end{multline}
where we set the weight term $w^{gp}$ to be $0.1$ for our experiments.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.485\textwidth]{figures/feature_loss.png}
    \caption{Feature loss illustration}
    \label{fig: feature}
\end{figure}

\subsection{Training of Generator} \label{sec:train_gen}
As we discussed, we train a generator to be natural and also to preserve the semantic features:
\begin{equation}
  \argmin_{G}\ \; w_{Na} L_{Na}(G) + w_{Fea}L_{Fea}(G),
\end{equation}
Where $L_{Na}$ is a naturalness loss and $L_{Fea}$ is a feature loss. We define $L_{Na}$ using our discriminator:
\begin{equation}
    L_{Na}(G) =  -log(D(G(\mathbf{x}^h_t, \mathbf{x}^r_{t-1}))),
\end{equation}
which encourages the generator to produce a natural latent variable. The feature loss $L_{Fea}$ is designed to match selected high level features:
The objective function 
\begin{align} \label{equ: eng_loss}
    L_{Fea}(G) &= || \Psi^h(\mathbf{x}^h_t)  - \Psi^r(\mathbf{x}^r_t) || \\ &=  || \Psi^h(\mathbf{x}^h_t)  - \Psi^r(\pi(G(\mathbf{x}^h_t, \mathbf{x}^r_{t-1}), \mathbf{x}^r_{t-1})) ||,
\end{align}
where $\Psi^h$ and $\Psi^r$ are manually designed the feature functions. The list of the features includes:
\begin{itemize}
  \item Height of the root
  \item Orientation of the root
  \item Linear and angular velocities of the root
  \item Offset from the shoulder to the elbow
  \item Offset from the elbow to the hand 
\end{itemize}
For all experiments, we set the values of $w_{Na}$ and $w_{Fea}$ to be 0.3 and 0.7. 

\subsection{Network Architecture}
Each generator G is modeled by neural network that maps given human motion state to a latent variable $\mathbf{z}_t = G(\mathbf{x}^p_t),\mathbf{x}^q_t))$. The network structure is a fully connected network with 2 hidden layers of [512, 512] units followed by learning output units. LeakyReLU activation are used for all networks. \sehoon{what about the discriminator?}

% \subsection{Sampling Algorithm}
% \input{algos/train_generator.tex}
% We train using Algorithm~\ref{algo:training}...
% \sehoon{Tianyu, please write a short paragraph that describes the key intuition of the algorithm.}











==> paper_text/ablation_study.tex <==
% \subsection{Ablation study}
% This section evaluates the impact on the performance with respect to adverserial and feature losses. The qualitative results are presented in the supplementary video.

% \subsubsection{Adversarial Loss} 
% In this experiment, we remove the adversarial loss $L_{disc}$ and retrain our network. We find that the framework fails to generate realistic motions with only the feature loss and motion prior. We suspect this is due to the inaccuracies of the trained motion prior, particularly on out-of-distribution data. In addition, the only-feature loss training can easily overlook the feasibility of the retargeted motion. One consequence is 
% self-collision. For instance, when the input human motion is lowering their hand, the optimal retargeted motion with the feature loss is the robot lowering its manipulator. However, for Spot the manipulator is mounted on its body, and lowering its manipulator by the same value as the human will result with self-penetration. The adversarial loss is helpful in reducing such cases, since there is no self-penetration in the character dataset.

% multiple latent variables can also lead to the same feature loss value, which causes ambiguity in the motion retargeting problem. This issue is critical when generating manipulator motion. For instance, the Spot manipulator has 8 joints, while the features only apply a on 6 DoF constraint. The 2 redundant DoF could lead to self-collision configurations. Adding the adversarial loss introduces constraints on the redundant DoF, forcing the generated motion to be similar to natural looking motion.



% In this experiment, we remove the adversarial loss $L_{Na}$ and retrain our network. We found that the framework fails to generate realistic motions with only the feature loss and motion prior. The main reason, in our opinion, is the modeling error of the motion prior. The adversarial loss controls the generated latent variable in the dataset's distribution. Once we remove this constraint, since the motion prior does not have good generalization properties when the latent variable is out of the distribution that the motion prior is trained on, other latent variables might also make the feature loss less. And these latent variables could not lead to realistic motions.

% \subsubsection{Feature Loss}
% In this experiment, we show the importance of the feature loss $L_{feat}$ by discarding it and retraining the networks. In this case, we observe mode collapse, and all human motions are retargeted to a single embedding that corresponds to a standing robot pose. This is not surprising because the standing motion does minimize the adversarial loss, and there are no other terms that force the generator to create diverse motions, reinforcing the importance of the feature loss - both for training stability and for preserving semantic knowledge of source motions.

% \subsection{Weights of the Loss} 
% The total loss for training the generator is defined as the sum of the weighted $L_{disc}$ and weighted $L_{feat}$. In this experiment, we aim to test how sensitive our method is to weight.
% We compared four sets of setting: $[w_{disc}, w_{feat}] = [0.7,0.3], \ [0.6, 0.4], \ [0.5, 0.5], \ [0.4, 0.6]$. The result shows all settings can retarget human motions to various robot natural-looking motions except when $[w_{disc}, w_{feat}]= [0.4, 0.6]$. In that setting, the self-collision rate reaches $9.21\%$, while the self-collision rate for other settings are $0.24 \%$ for [0.7,0.3], $0.8 \%$ for [0.6,0.4], and $1.96 \%$ for [0.5,0.5]. Thus, we may conclude that our method is not extremely sensitive to hyperparameters, but reducing the weight on $L_{disc}$ can result in physically unrealistic motions.


%One potential solution can be maximizing the entropy term used by \cite{}; however, we will leave this as future work.
% In this experiment, we show the effectiveness of the feature loss $L_{Fea}$ by discarding it and retraining the network. From our result, without the feature loss, all motions are retargeted to a single latent variable that leads to a standing pose. This result is unsurprising since the standing motion does minimize the adversarial loss, and there is no other term that could trigger generating different latent variables from different input human motions. One potential candidate could be maximizing entropy term used by \cite{}, however, we will leave this to our future work.

% \subsubsection{Feature Loss on the Embedded Space}
% In this work, we assume the embedded latent space is provided beforehand to ensure the quality of the pretrain motion prior such that it wouldn't affect the overall performance of our framework. In this experiment, we did ablation on designing feature loss on the latent space. Here the new feature loss can be formulated as follows:
% \begin{equation}
%     L'_{feat}(G) = || \Psi^p(\mathbf{x}^p_t)  - \Psi'^q(\mathbf{z}^q_t) || =  || \Psi^p(\mathbf{x}^p_t)  - \Psi^q(G(\mathbf{x}^p_t, \mathbf{x}^q_{t-1})) ||
%     \label{equ: new_eng_loss}
% \end{equation}

% \akshara{Is the first input $x$ or $z$? Why are we comparing the features on state to latent space? }
% \akshara{I don't follow this experiment - maybe remove for now, or add to appendix, especially since the result does not show a difference?}
%  the result shows no significantly different between trained with the predicted state(our original method) and trained with the embedded state(this ablation). This indicates that our motion prior is trained properly such that it can predict an accurate state. It also demonstrates that if we have access to the high-level state, we can do learning on the high-level space. \sehoon{Tianyu, I don't follow the logic here. 1) How do you compute $\Psi'^q$ from the latent value? 2) What is the meaning of this experiment, if it makes no difference?}
%  \tianyu{The logic is: comparing our work (feature loss on the low level predicted state) with feature loss on latent space. We want to show that if the latent space is explainable, it's possible to do feature loss on the high level space. However, in most cases the latent space is unexplainable, so 'feature loss on latent space' is not possible.Maybe I can try another ablation study?} \sehoon{I am not sure this ablation is super necessary}



==> paper_text/background.tex <==
\section{Background}
\tianyu{Not sure if should add a section to overview some preknowledge}

\subsection{Adversarial learning for motion retargeting}

==> paper_text/human_data.tex <==
\section{Human Motion Data Preparation} \label{sec:human_data}
First, we prepare a human motion dataset $\Omega^h =\{ \xi_0:(\mathbf{x}^h_1, \mathbf{x}^h_2, \cdots, \mathbf{x}^h_N ), \xi_1, \cdots, \xi_{N'} \}$ that serves as an input distribution to adversarial learning. Here $\xi_i$ denotes a single human motion trajectory containing state sequence $(\mathbf{x}^h_1, \mathbf{x}^h_2, \cdots, \mathbf{x}^h_N)$. Each trajectory can have a different length of state sequence depending on the source motion. The motion state $\mathbf{x}^h_i$ includes features as follows:
\begin{itemize}
  \item Height of the root from the ground (1 dim)
  \item Rotation of the root (4 dims) 
  \item Linear and angular velocities of the root (6 dims)
  \item Left and Right Shoulder position (3 or 6 dims)
  \item Left and Right Elbow position (3 or 6 dims)
  \item Left and Right Wrist position (3 or 6 dims)
\end{itemize}
Except for the height of the root, all the features are defined in the \emph{local coordinate} frame of the character. Specifically, we define the local coordinate frame as follows. First, we select the pelvis of the character as the root node. Then the character's local coordinate frame is defined with its origin on the root node, its x-axis aligned with the direction that the character is facing and its z-axis is aligned with a global vertical vector. This defines a $20$ dimensional feature space for one-handed motions (e.g., for single manipulator robots) and a $29$ dimensional feature space for two-handed motions (e.g., for double manipulators robot). 
\sehoon{Tianyu, we can show a figure with a character and their features here} \akshara{good to visualize the frame of reference at least.}



% The human motion state $\mathbf{x}^p_t$ consists of a set of features that describes the configuration of the human at time t. The features include:
% \begin{itemize}
%   \item Height of root of human from the ground
%   \item Rotation of the root of human in local coordinate frame
%   \item Linear and angular velocity of the root in local coordinate frame
%   \item Shoulder position in local coordinate frame
%   \item Elbow position in local coordinate frame
%   \item Wrist position in local coordinate frame
% \end{itemize}
% The root is designated to be the human character's pelvis. The character's local cordinate frames is defined as the origin located at root, the x-axis oriented the chracter's facing direction and the z-axis are aligned with global vertical vector.


==> paper_text/motion_prior.tex <==
\section{Pre-training of Robot Motion Prior} \label{sec:motion_prior}
In this section, we will describe the training process of robot motion prior $\pi(\mathbf{z}_{t}, \mathbf{x}^r_{t-1}) \mapsto \mathbf{x}^r_t$, which maps the latent variable $\mathbf{z}_{t}$ and the previous character's state $\mathbf{x}^r_{t-1}$ to the character's state at the current step $\mathbf{x}^r_{t}$. Standard motion retargeting algorithms often directly map the given input motion of the source character to a high-dimensional motion of the target character. However, learning such a complex mapping can be less practical because it leads to unstable convergence during training. Instead, we decided to train a motion prior that controls the robot's motion based on a compact latent command, which makes the learning of the mapping much easier. We interpret this process as using the generator to infer a task/skill, and the target character uses its own way (motion prior) to accomplish the same task/skill. 














Therefore, the key to successful motion retargeting is to learn an expressive motion prior that can execute a large range of motor skills. For this purpose, we learn two motion priors for locomotion and manipulation by decoupling upper and lower body motions instead of learning a single motion prior. This design decision makes the training of motion prior much easier and also reduces the amount of the required dataset. Please note that this does not mean that we treat upper and lower body motions separately: we still aim to learn natural whole-body motions at the stage of adversarial learning.

In the following sections, we will discuss design choices for learning robot motion prior.

\subsection{Robot Motion Data Preparation}
% We build locomotion and manipulation motion datasets for each robot. We generate the locomotion of legged robots (Spot and Daisy) by solving a simple motion planning algorithm [cite] \sehoon{do we have any reference?} with randomly sampled target linear and angular velocities in the range of [XXX, XXX] m/s and [XXX, XXX] rad/s. The gait, such as walking, trotting, and galloping, is selected based on the magnitude of the target speed. For the wheeled robot (Stretch), we move its base with the given target velocity commands. For manipulation, we randomly select the target positions and solve inverse kinematics problems while filtering out poses with self-collisions. We enforce continuity of manipulation data by ... \sehoon{any thoughts?}.

\tianyu {I prefer not to talk too detail about the dataset,  our framework should be agnostic to dataset and robots. To show the framework is general, I would not to mention any specific robot in this section }

The robot locomotion and manipulation dataset is build 


\subsection{State and Command Spaces}
Once the robot motions are prepared, we construct a robot motion data set $\Omega^r = \{\mathbf{x}^r_1, \mathbf{z}^r_1, \mathbf{x}^r_2, \mathbf{z}^r_2, \cdots, \mathbf{x}^r_M\}$, where $\mathbf{x}^r_1$ and $\mathbf{z}$ represent a state feature vector and a latent command vector. Because we decouple the locomotion and manipulation motion priors, we prepare two separate datasets: a locomotion dataset $\Omega^{r,L}$ and a manipulation dataset $\Omega^{r,M}$. 

\subsubsection{Locomotion State Spaces}
The features of locomotion include the following items:
\begin{itemize}
  \item Height of the root from the ground ($1$ dim)
  \item Orientation of the root ($4$ dim)
  \item Relative location of the root from the previous frame ($2$ dim) 
  \item Relative orientation of the root from the previous frame ($4$ dim) 
  \item Linear and angular velocities of the root ($6$ dim)
  \item Foot position ((3 * Number of foot) dim)
  \item Foot velocities ((3 * Number of foot) dim)
  \item Phase variable ($1$ dim)
\end{itemize}
Similar to Section~\ref{sec:human_data}, the features are defined in the \emph{local frame}, which is centered at the root node. The phase variable is a scalar value $\in [0,1)$ growing linearly as a function of time from 0 to 1, and reset to 0 when it reaches 1. \sehoon{how much do you add per frame?}\tianyu{I don't think it's necessary to mention that. In fact, for each controller, the rate is even different. Since it's in the dataset, the increasing rate can be learned} 
% This defines a $XXX$ dimensional feature space for Spot, a $XXX$ dim space for Daisy, and a $XXX$ dim space for Stretch. 

\subsubsection{Locomotion Command Spaces}
We also extract latent commands from the motions, which will be used when we train motion priors. From two consecutive frames, we extract the following commands:
\begin{itemize}
  \item Desired height of the root from the ground in the next frame ($1$ dim)
  \item Desired linear and angular velocities of the root ($6$ dim)
\end{itemize}
The last item, the desired linear and angular velocities of the root, is computed using the finite difference. This results in a $7$ dimensional command vector.

\subsubsection{Manipulation State Spaces}
Inspired by the idea of the group of body parts(GBP) \cite{delhaisse2017transfer}, we define the features for manipulation as:
\begin{itemize}
  \item Joint angles of the manipulator
  \item Cartesian positions of key joints
\end{itemize}
All the quantities are defined in the robot's local coordinate frame. Key joints are manually picked by an expert, as illustrated in Figure \ref{fig: feature}. Although joint angles and key joint positions are redundant in the sense that we can calculate key joint positions in Cartesian coordinates using forward kinematics, we found that this redundancy does not harm the learning and makes our system easier to implement. 
% As a result, it defines $XXX$ dim, $XXX$ dim, and $XXX$ dim state space for Spot, Daisy, and Stretch robots, respectively.

\subsubsection{Manipulation Command Spaces}
Finally, the command vector for manipulation is defined as:
\begin{itemize}
  \item Desired Cartesian positions of key joints
\end{itemize}
which yields a $XXX$ dimensional vector.

\subsection{Training of Motion Prior}
Once we obtain two datasets $\Omega^{r, L}$ and $\Omega^{r, M}$, we can train a motion prior that takes as inputs the low-dimensional control embedding and the current pose and predicts the next pose. Recent literature~\cite{VAEs, ASE, zhang2018mode, abdul2017motion} in computer animation has discussed learning-based techniques to obtain such kinematic controllers. Notably, our framework is agnostic to the choice of the method. Here, we train a motion prior $\pi^L$ and $\pi^M$ using supervised learning:
\begin{equation} \label{equ:supervised_learning}
    \argmin_{\pi}\  \mathbb{E}_{(\mathbf{x}^r_{t-1},\mathbf{z}^r_{t-1},\mathbf{x}^r_{t}) \backsim \Omega^r} ||\mathbf{x}^r_{t} - \pi(\mathbf{z}_{t-1}, \mathbf{x}^r_{t-1})||
\end{equation}
where $\mathbf{x}^r_t$ are the robot state at time instant t, $\mathbf{z}_t$ is the latent control embedding. We assume all these terms are available in the dataset $\Omega^r$ as the learning method is independent of the paper's focus. Because we decouple the motion of locomotion (root and leg motions) and manipulation (arm motions), we repeat the optimization (Equation~\ref{equ:supervised_learning}) twice for $(\pi^L, \omega^L)$ and $(\pi^M, \omega^M)$ to train controllers separately. Once we obtain $\pi^L$ and $\pi^M$, we can stack their states and latent variables to obtain a single controller $\pi(\mathbf{z}_{t-1}, \mathbf{x}^r_{t-1}) \mapsto \mathbf{x}^r_t$.


\subsection{Mixture of Experts Architecture}
Our locomotion dataset contains three different gaits, walking, trotting, and galloping, with different target velocities. This large diversity of the motion often deteriorates the accuracy of the motion prior, which causes awkward foot penetration or foot skating effects. To this end, we adopt the mixture of expert (MOE) architecture, which combines the predictions of multiple motion priors (experts) to make a final prediction. We manually cluster the motion data into different subsets based on its gait and train experts on the corresponding subsets. We also augment the latent variable $\mathbf{z}$ with a three-dimensional one-hot vector that selects the proper expert. In our experience, the MOE architecture greatly improves the quality of the generated locomotion. On the other hand, we still train a single expert for the manipulation motion prior.


